Target Conditioning for One-to-Many Generation

Neural Machine Translation (NMT) models often lack diversity in their generated translations, even when paired with search algorithm, like beam search. A challenge is that the diversity in translations are caused by the variability in the target language, and cannot be inferred from the source sentence alone. In this paper, we propose to explicitly model this one-to-many mapping by conditioning the decoder of a NMT model on a latent variable that represents the domain of target sentences. The domain is a discrete variable generated by a target encoder that is jointly trained with the NMT model. The predicted domain of target sentences are given as input to the decoder during training. At inference, we can generate diverse translations by decoding with different domains. Unlike our strongest baseline (Shen et al., 2019), our method can scale to any number of domains without affecting the performance or the training time. We assess the quality and diversity of translations generated by our model with several metrics, on three different datasets.

==> content/old.tex <==

% \begin{table}
% \centering
% \begin{tabular}{l|cc}
%     \toprule
%     & \mbleu & \pairwise \\
%     \midrule
%     $\lambda=0$  & - & - \\
%     $\lambda=3$  & - & - \\
%     $\lambda=10$ & - & - \\
%     $\lambda=50$ & - & - \\
%     \bottomrule
% \end{tabular}
% \caption{Results for WMT En-De for $\ndomain=10$ target domains for our method with different values of $\lambda$.}
% \label{tab:ablation_entropy}
% \end{table}

% \begin{table}
% \centering
% \begin{tabular}{l|cc}
%     \toprule
%     & \mbleu & \pairwise \\
%     \midrule
%     $T=0.1$ & - & - \\
%     $T=0.3$ & - & - \\
%     $T=1$   & - & - \\
%     $T=3$   & - & - \\
%     $T=10$  & - & - \\
%     \bottomrule
% \end{tabular}
% \caption{Results for WMT En-De for $\ndomain=10$ target domains for our method with different temperature values.}
% \label{tab:ablation_temperature}
% \end{table}


% Target sentences are encoded with a transformer target encoder. The first hidden state of the last layer is linearly mapped to a vector of scores $s \in \mathcal{R}^{\ndomain}$, on which we apply a softmax layer to get a vector $p \in \mathcal{R}^{\ndomain}$. We compute the first embedding $e$ given as input to the decoder with:

% At inference time, a source sentence is encoded, and $\ndomain$ translations are generated by providing the different $e_i$ to the decoder.
% In practice, we also apply a temperature on the domain scores $s$, that decreases linearly from 1 to 0 over training. When the temperature reaches 0, the target encoder does not receive any gradient as computing $p$ is equivalent to applying an $\argmax$ operator.
% , which amounts to feeding a first embedding $\sum_{i=0}^{\ndomain-1}{p_i e_i}$ where $p$ is a one-hot vector
%  (i.e. the decoder is trained with vectors $p \in \mathcal{R}^\ndomain$ summing to $1$, and at test time $p$ is a one-hot vector)

% The smaller T, the closer to argmax is the softmax with temperature.
% Finally, to obtain the target latent variable $u$, we compute:
% $$u = \sum_{i=0}^{K}{p_ie_i}$$
% where $(e_0,..,e_{K-1})$ are K embedding vectors of dimension H, that represent our K domains. These embeddings are learned during training. We alternate between softmax and argmax because the softmax makes possible to have gradients and argmax gives one-hot vector for $u$ which is what we have at inference time.\\
% Parallely, the source sentence is encoded through a bi-directional transformer of size size L=6, H=512, A=8.\\

% to obtain the target logits $l$.
% According to a probability $\alpha$, we either apply a argmax function or a softmax function with a temperature $T>0$, on the logits to obtain the target probability $p$.

% A possible issue could be that independently of the input target sentence. We refer to this phenomenon as ``mode dropping''.
% a implementation of the proposed method can lead to a collapse where the target encoder only predicts one domain.

